Circuit complexity, proof complexity, and polynomial identity testing

We introduce a new algebraic proof system, which has tight connections to (algebraic) circuit complexity. In particular, we show that any super-polynomial lower bound on any Boolean tautology in our proof system implies that the permanent does not have polynomial-size algebraic circuits (VNP is not equal to VP). As a corollary to the proof, we also show that super-polynomial lower bounds on the number of lines in Polynomial Calculus proofs (as opposed to the usual measure of number of monomials) imply the Permanent versus Determinant Conjecture. Note that, prior to our work, there was no proof system for which lower bounds on an arbitrary tautology implied any computational lower bound. Our proof system helps clarify the relationships between previous algebraic proof systems, and begins to shed light on why proof complexity lower bounds for various proof systems have been so much harder than lower bounds on the corresponding circuit classes. In doing so, we highlight the importance of polynomial identity testing (PIT) for understanding proof complexity. More specifically, we introduce certain propositional axioms satisfied by any Boolean circuit computing PIT. We use these PIT axioms to shed light on AC^0[p]-Frege lower bounds, which have been open for nearly 30 years, with no satisfactory explanation as to their apparent difficulty. We show that either: a) Proving super-polynomial lower bounds on AC^0[p]-Frege implies VNP does not have polynomial-size circuits of depth d - a notoriously open question for d at least 4 - thus explaining the difficulty of lower bounds on AC^0[p]-Frege, or b) AC^0[p]-Frege cannot efficiently prove the depth d PIT axioms, and hence we have a lower bound on AC^0[p]-Frege. Using the algebraic structure of our proof system, we propose a novel way to extend techniques from algebraic circuit complexity to prove lower bounds in proof complexity.

==> intro.tex <==
\begin{abstract}
We introduce a new and very natural algebraic proof system, which has tight connections to (algebraic) circuit complexity. In particular, we show that any super-polynomial lower bound on any Boolean tautology in our proof system implies that the permanent does not have polynomial-size algebraic circuits ($\cc{VNP} \neq \cc{VP}$). Note that, prior to our work, there was no proof system for which lower bounds on an arbitrary tautology implied \emph{any} computational lower bound. 

Our proof system helps clarify the relationships between previous algebraic proof systems, and begins to shed light on why proof complexity lower bounds for various proof systems have been so much harder than lower bounds on the corresponding circuit classes. In doing so, we highlight the importance of polynomial identity testing (PIT) for understanding proof complexity.

More specifically, we introduce certain propositional axioms satisfied by any Boolean circuit computing PIT. (The existence of efficient proofs for our PIT axioms appears to be somewhere in between the major conjecture that PIT$\in \cc{P}$ and the known result that PIT$\in \cc{P/poly}$.) We use these PIT axioms to shed light on $\cc{AC}^0[p]$-Frege lower bounds, which have been open for nearly 30 years, with no satisfactory explanation as to their apparent difficulty. We show:
\begin{enumerate}
\item Either proving superpolynomial lower bounds on $\cc{AC}^0[p]$-Frege implies $\cc{VP}_{\F_p} \neq \cc{VNP}_{\F_p}$, thus explaining the difficulty of lower bounds on $\cc{AC}^0[p]$-Frege, or

\item $\cc{AC}^0[p]$-Frege cannot efficiently prove the PIT axioms, and hence we have a lower bound on $\cc{AC}^0[p]$-Frege.
\end{enumerate}
We also get a similar statement relating our PIT axioms for depth $d+2$ algebraic circuits, lower bounds on depth $d$ $\cc{AC}^0_d[p]$-Frege, and the statement that $\cc{VNP}_{\F_p}$ does not have polynomial size depth $d+2$ algebraic circuits (the latter being notoriously beyond our current techniques for any $d > 1$)

%We get similar statements regarding a) depth 4 PIT axioms and $2^{\omega(\sqrt{n} \log n)}$ lower bounds on depth $d$ $\cc{AC}^0$-Frege---another problem that has been open for nearly 30 years with seemingly no explanation for its difficulty---and b) depth $d+2$ PIT axioms and super-polynomial lower bounds on depth $d$ $\cc{AC}^0$- or $\cc{AC}^0[p]$-Frege.

Finally, using the algebraic structure of our proof system, we propose a novel way to extend techniques from algebraic circuit complexity to prove lower bounds in proof complexity. Although we have not yet succeeded in proving such lower bounds, this proposal should be contrasted with the difficulty of extending $\cc{AC}^0[p]$ circuit lower bounds to $\cc{AC}^0[p]$-Frege lower bounds.

%this result scales down to $\cc{AC}^0$-Frege and to $\cc{AC}^0[p]$-Frege, where we 

%[TODO] This allows us to give a new, self-contained, and simpler proof that $\cc{NP} \not\subseteq \cc{coMA}$ implies the permanent does not have polynomial-size constant-free circuits ($\cc{VNP}^0 \neq \cc{VP}^0$). Our proof system also has the advantage that it begins to make clear and precise how much harder it is to prove lower bounds in algebraic proof complexity than in algebraic circuit complexity. It thus helps explain why it has been so difficult to prove true size (=length-of-proof) lower bounds on algebraic proof systems, and thereby also lower bounds on $\cc{AC}^0[p]$-Frege systems (an open problem for 30+ years). Finally, we flip this difference in hardness on its head, to suggest a new way to transfer techniques from algebraic proof complexity, such as the method of partial derivatives, to prove lower bounds in algebraic proof complexity.
\end{abstract}

\section{Introduction}
$\cc{NP}$ versus $\cc{coNP}$ is the very natural question of whether, for every graph that doesn't have a Hamiltonian path, there is a short proof of this fact. One of the arguments for the utility of proof complexity is that by proving lower bounds against stronger and stronger proof systems, we ``make progress'' towards proving $\cc{NP} \neq \cc{coNP}$. However, until now this argument has been more the expression of a philosophy or hope, as there is no known proof system for which lower bounds imply computational complexity lower bounds of any kind, let alone $\cc{NP} \neq \cc{coNP}$.

We remedy this situation by introducing a very natural algebraic proof system, which has tight connections to (algebraic) circuit complexity. We show that any super-polynomial lower bound on any Boolean tautology in our proof system implies that the permanent does not have polynomial-size algebraic circuits ($\cc{VNP} \neq \cc{VP}$). Note that, prior to our work, essentially all implications went the opposite direction: a circuit complexity lower bound implying a proof complexity lower bound. 

We show that under a reasonable assumption on PIT, our proof system is p-equivalent to Extended Frege, the strongest-known natural propositional proof system. 
In combination with the above result, this helps explain why obtaining lower bounds on Extended Frege has been so difficult. More specifically, we hypothesize that Extended Frege can efficiently prove certain propositional axioms satisfied by any Boolean circuit computing PIT (this hypothesis appears to be somewhere in between the major hypothesis that PIT$\in \cc{P}$ and the known result that PIT$\in \cc{P/poly}$). Note that, although PIT has played an increasingly prominent role in circuit complexity and algorithms, until now it has been almost entirely absent from the setting of proof complexity.


We also highlight the importance of our PIT axioms for understanding lower bounds on $\cc{AC}^0[p]$-Frege, which have been open for nearly 30 years, despite having the corresponding $\cc{AC}^0[p]$ circuit lower bounds. We show:
\begin{enumerate}
\item Either proving superpolynomial lower bounds on $\cc{AC}^0[p]$-Frege implies $\cc{VP}_{\F_p} \neq \cc{VNP}_{\F_p}$, thus explaining the difficulty of lower bounds on $\cc{AC}^0[p]$-Frege, or

\item $\cc{AC}^0[p]$-Frege cannot efficiently prove the PIT axioms, and hence we have a lower bound on $\cc{AC}^0[p]$-Frege.
\end{enumerate}
We get similar statements regarding a) depth 4 PIT axioms and $2^{\omega(\sqrt{n} \log n)}$ lower bounds on depth $d$ $\cc{AC}^0$-Frege---another problem that has been open for nearly 30 years with seemingly no explanation for its difficulty---and b) depth $d+2$ PIT axioms, super-polynomial lower bounds on depth $d$ $\cc{AC}^0$- or $\cc{AC}^0[p]$-Frege, and super-polynomial lower bounds on depth $d+2$ algebraic circuits for the permanent.

We get a similar dichotomy between truly exponential ($2^{\omega(\sqrt{n} \log n)}$) depth $d$ $\cc{AC}^0$-Frege lower bounds---another 30-year-open question with seemingly no explanation for its difficulty---and polynomial-size $\cc{AC}^0_d$-Frege proofs of the depth 4 version of our PIT axioms.

Finally, using the algebraic structure of our proof system, we propose a novel way to extend techniques from algebraic circuit complexity to prove lower bounds in proof complexity. Although we have not yet succeeded in proving such lower bounds, this proposal should be contrasted with the difficulty of extending $\cc{AC}^0[p]$ circuit lower bounds to $\cc{AC}^0[p]$-Frege lower bounds.

\subsection{Background and Motivation}
\paragraph{Algebraic Circuit Complexity.} The most natural way to compute a polynomial function $f(x_1,\ldots,x_n)$ is
with an algebraic circuit, where the input consists of the variables $x_1,\ldots,x_n$,
and the computation is performed
using the arithmetic operations: addition, multiplication and subtraction.
The ultimate goal is to understand the optimal complexity, in terms of size and depth,
of computing a given polynomial family.
The importance of the arithmetic circuit model was increased by several
results of Valiant \cite{valiant,valiantPerm,valiantProjections}, who
argues that understanding
arithmetic circuits is very important, not only because they are
interesting in themselves, but also because that understanding may
give new intuitions
that may be used for the understanding of
other models of computation. (See also \cite{Gat2}.)

Two central functions in this area are the determinant and permanent polynomials, 
which are fundamental because of their prominent role in many areas of mathematics,
and in addition they are known to be complete
for the classes $\cc{VP}$ and $\cc{VNP}$ respectively.
$\cc{VP}$ and $\cc{VNP}$ can be viewed as algebraic analogs of the complexity classes
$\cc{P}$ and $\cc{NP}$, respectively,\footnote{It is somewhat more accurate to say that $\cc{VP}$ is the algebraic analog of $\cc{FNC}^2$ $\cc{VNP}$ is the algebraic analog of $\cc{\# P}$.} and thus a major open problem is to
show that $\cc{VP} \neq \cc{VNP}$, or in other words, that the permanent cannot
be computed by arithmetic circuits of polynomial size, thus resolving
an algebraic analog of the $\cc{P}$ versus $\cc{NP}$ question. 

Unlike in Boolean circuit complexity,
non-trivial lower bounds
for the size of arithmetic circuits
are known (proven in the seminal papers of Strassen
and Baur--Strassen \cite{strassenDegree,baurStrassen}).
Their methods, however, only give lower bounds of
up to
$\Omega (n\log n)$.
Moreover, their methods are based on  a degree analysis
of certain algebraic varieties and do not give  lower bounds for
polynomials of constant degree.
Recent exciting work [REF] has shown that polynomial-size algebraic
circuits can in fact be computed by subexponential-size depth 4 algebraic
circuits. 
Thus, strong enough lower bounds for depth 4 arithmetic circuits for
the permanent would already prove $\cc{VP} \neq \cc{VNP}$.
Recently work shows that this problem is essentially equivalent
to another major open problem in complexity theory,
obtaining a deterministic, polynomial-time algorithm for
polynomial identity testing.
(or to the derandomization of of all Boolean polynomial-time computations.?)

\medskip

\paragraph{Proof Complexity.} One of the most basic questions of logic is the following: given a tautology, what is the
length of the shortest proof of the statement in some standard axiomatic proof system? This question inspired Cook's
seminal paper on $\cc{NP}$-completeness \cite{cook:np} and were contemplated even earlier by \Godel in his now
well-known letter to von Neumann (see \cite{buss:kprov}). The propositional version of this question, whether there exists a propositional proof system giving rise to short proofs of all tautologies, is equivalent to the central question in complexity theory  of whether $\cc{NP}$ equals $\cc{coNP}$ \cite{cookReckhow}. In this same line of work, they proposed a research program
of proving super-polynomial lower bounds for increasingly powerful standard proof systems. However, despite considerable progress obtaining superpolynomial lower bounds for many weak proof systems (resolution, cutting planes,
bounded-depth Frege systems), there has been essentially no progress in the last 25 years for stronger proof systems such as Extended Frege systems or Frege systems.
More surprisingly, proving nontrivial lower bounds for $\cc{AC}^0[p]$-Frege systems is still unresolved.
Note that in contrast, the analogous result in circuit complexity (proving  superpolynomial $\cc{AC}^0[p]$ lower bounds for an explicit function) was resolved by Smolensky over 25 years ago \cite{smolensky}.

To date, there has been no satisfactory explanation for this state of affairs.
In proof complexity, there are no known formal barriers such as relativization \cite{bakerGillSolovay}, Razborov--Rudich natural proofs \cite{razborovRudich}, or algebrization \cite{aaronsonWigderson} that exist in Boolean function complexity.
Moreover, there has not even been progress by way of conditional
lower bounds. That is, trivially $\cc{NP} \neq \cc{coNP}$ implies superpolynomial
lower bounds for $\cc{AC}^0[p]$-Frege, but we know of no weaker complexity assumption
that implies such lower bounds.
The only formal implication in this direction shows that certain
circuit lower bounds imply lower bounds for proof systems that admit
feasible interpolation, but unfortunately only weak proof systems
(not Frege nor even $\cc{AC}^0$-Frege) have this property \cite{Bonet,Bonet2}.
In the converse direction, there are essentially no implications
at all. For example, we do not know if $\cc{AC}^0[p]$-Frege
lower bounds (nor even Frege nor Extended Frege lower bounds) imply any
nontrivial circuit lower bounds.

\subsection{Our Results}
In this paper, we define a simple and natural proof system that we call the Ideal Proof System (IPS)
based on Hilbert's Nullstellensatz. Our system is similar in spirit to related
algebraic proof systems that have been previously studied, but is different in a crucial way (explained below).

Given a set of polynomials $F_1,\ldots,F_m$ in $n$ variables $x_1,\ldots,x_n$ over a field $\F$ without a
common zero over the algebraic closure of $\F$, Hilbert's Nullstellensatz says that there exist polynomials
$G_1,\ldots,G_m \in \F[x_1,\ldots,x_n]$ such that $\sum F_i G_i =1$, \ie, that $1$ is in the ideal generated by the $F_i$. In the Ideal Proof System, we introduce new variables $\f_i$ which serve as placeholders into which the original polynomials $F_i$ will
eventually be substituted:

\begin{definition}[Ideal Proof System] \label{def:IPS}
An \definedWord{\I certificate} that a system of $\F$-polynomial equations
$F_1(\vec{x})=F_2(\vec{x}) = \dotsb = F_m(\vec{x}) = 0$ is unsatisfiable over $\overline{\F}$ is
a polynomial $C(\vec{x}, \vec{\f})$ in the variables $x_1,\ldots,x_n$ and $\f_1,\ldots,\f_m$ such that
\begin{enumerate}
\item \label{condition:ideal} $C(x_1,\dotsc,x_n,\vec{0}) = 0$, and
\item \label{condition:nss} $C(x_1,\dotsc,x_n,F_1(\vec{x}),\dotsc,F_m(\vec{x})) = 1$.
\end{enumerate}
The first condition is equivalent to $C$ being in the ideal generated by $\f_1, \dotsc, \f_m$, and the two conditions together therefore imply that $1$ is in the ideal generated by the $F_i$, and hence that $F_1(\vec{x}) = \dotsb = F_m(\vec{x})=0$ is unsatisfiable. 

An \definedWord{\I proof} of the unsatisfiability of the polynomials $F_i$ is
an $\F$-algebraic circuit on inputs $x_1,\ldots,x_n,\f_1,\ldots,\f_m$ computing some algebraic
certificate of unsatisfiability.
\end{definition}

For any class of algebraic circuits $\mathcal{C}$, we may speak of $\mathcal{C}$-\I proofs of a family of systems of equations $(\mathcal{F}_n)$ where $\mathcal{F}_n$ is $F_{n,1}(\vec{x}) = \dotsb = F_{n,\poly(n)}(\vec{x}) = 0$. When we refer to \I without further qualification, we mean $\cc{VP}$-\I, that is, the family of \I proofs should be computed by circuits of polynomial size \emph{and polynomial degree}, unless specified otherwise.

Like previously defined algebraic systems \cite{BIKPP,CEI,pitassi96,pitassiICM}, proofs in our system can be
checked in randomized polynomial time.
The key difference between our system and previously studied
ones is that those systems are axiomatic in the sense that they require that \emph{every}
subcomputation (derived polynomial) be in the ideal generated by the original polynomial equations $F_i$, and thus be a sound consequence of the equations $F_1=\dotsb=F_m=0$.
In contrast our system has no such requirement; an \I proof can compute potentially
unsound subcomputations (whose vanishing does not follow from $F_1=\dotsb=F_m=0$), as long as the \emph{final polynomial} is in the ideal
generated by the equations. This key difference allows \I proofs to be
\emph{ordinary algebraic circuits}, and thus nearly all results in
algebraic circuit complexity apply directly to the Ideal Proof System. To quote the tagline of a common US food chain, the Ideal Proof System is a ``No rules, just right'' proof system.

Our first main theorem shows one of the advantages of this close connection with algebraic circuits. To the best of our knowledge, this is the first implication showing that a proof complexity lower bound implies any sort of computational complexity lower bound. 

\begin{VNPthm}
Superpolynomial lower bounds for the Ideal Proof System imply that the permanent does not have polynomial-size
algebraic circuits, that is, $\cc{VNP} \neq \cc{VP}$.
\end{VNPthm}

\begin{comment:parityP}
As a simple corollary, we obtain a very different and arguably simpler proof
of the following result: 

\begin{corollary}
If $\cc{NP}$ is not contained in $\cc{coMA}$, then $\cc{\parity P/poly}$ is not equal to $\cc{NC^1/poly}$.
\end{corollary}
\end{comment:parityP}

%In Section~\ref{sec:others}, we address the power of \I relative to standard proof systems. We show that \I can simulate Extended Frege systems, and similarly, subsystems of \I can simulate the corresponding subsystems of Extended Frege systems. More surprisingly, we prove the following conditional result in the other direction, that Extended Frege can polynomially-simulate the Ideal Proof System under a reasonable assumption about polynomial identity testing (PIT).

Under a reasonable assumption on polynomial identity testing (PIT), which we discuss further below, we are able to show that Extended Frege is equivalent to the Ideal Proof System. Extended Frege (EF) is the strongest natural deduction-style propositional proof system that has been proposed, and the proof complexity analog of $\cc{P/poly}$ (that is, Extended Frege = $\cc{P/poly}$-Frege). 

\begin{EFthm}
Let $K$ be a family of polynomial-size Boolean circuits for PIT such that the PIT axioms for $K$ (see Definition~\ref{def:PITaxioms}) have polynomial-size EF proofs. Then EF polynomially simulates \I, and hence the EF and \I are polynomially equivalent.
\end{EFthm}

Under this assumption about PIT, Theorems~\ref{thm:VNP} and \ref{thm:EF} in combination suggest a precise reason that proving lower bounds on Extended Frege is so difficult, namely, that doing so implies $\cc{VP} \neq \cc{VNP}$. Theorem~\ref{thm:EF} also suggests that to make progress toward proving lower bounds in proof complexity, it may be necessary to prove lower bounds for the 
Ideal Proof System, which we feel is more natural, and creates the possibility of harnessing tools from algebra, representation theory, and algebraic circuit complexity. We give a specific suggestion of how to apply these tools towards proof complexity lower bounds in Section~\ref{sec:syzygy}.

\begin{remark}
Given that $PIT \in \cc{P}$ is known to imply lower bounds, one may wonder if the combination of the above two theorems really gives any explanation at all for the difficulty of proving lower bounds on Extended Frege. There are at least two reasons that it does. 

First, the best known lower bound that follows from $PIT \in \cc{P}$ is an algebraic circuit-size lower bound on an integer polynomial that is computable in $\cc{NE} \cap \cc{coNE}$, whereas our conclusion is a lower bound on algebraic circuit-size for a function in $\cc{\# P} \subseteq \cc{PSPACE}$. 

Second, the hypothesis that our PIT axioms can be proven efficiently in Extended Frege seems to be somewhat orthogonal to, but likely no stronger than, the widely-believed hypothesis that PIT is in $\cc{P}$. As Extended Frege is a nonuniform proof system, efficient Extended Frege proofs of our PIT axioms are unlikely to have any implications about the uniform complexity of PIT (and given that we already know unconditionally that PIT is in $\cc{P/poly}$, uniformity is what the entire question of derandomizing PIT is about). In the opposite direction, we note that under a standard working hypothesis in proof complexity, if PIT is in $\cc{P}$, then our PIT axioms can indeed be efficiently proven in Extended Frege (see Remark~\ref{rmk:PITproof} for details). \rmkqed
\end{remark}


%Unlike in circuit complexity, however, there are almost no examples of tautologies that are even conjectured to be hard to prove in Extended Frege (see \cite{} for some of the only known conjectures), let alone any nontrivial lower bounds.  Furthermore, our next main theorem shows that, under a reasonable assumption on polynomial identity testing (PIT), our system is equivalent to Extended Frege, th

Although PIT has long been a central problem of study in computational complexity---both because of its importance in many algorithms, as well as its strong connection to circuit lower bounds---our theorems highlight the importance of PIT in proof complexity. Next we prove that Theorem~\ref{thm:EF} can be scaled down to obtain similar resuls for weaker Frege systems, and discuss some of its more striking consequences.

\begin{AC0thm}
Let $\mathcal{C}$ be any of the standard circuit classes $\cc{AC}^k, \cc{AC}^k[p], \cc{ACC}^k, \cc{TC}^k, \cc{NC}^k$. Let $K$ be a family of polynomial-size Boolean circuits for PIT (not necessarily in $\mathcal{C}$) such that the PIT axioms for $K$ have polynomial-size $\mathcal{C}$-Frege proofs. Then $\mathcal{C}$-Frege is polynomially equivalent to \I, and consequently to Extended Frege as well.
\end{AC0thm}

Theorem~\ref{thm:AC0} also highlights the importance of our PIT axioms for getting $\cc{AC}^0[p]$-Frege lower bounds, which has been an open question for more than thirty years. (For even weaker systems, Theorem~\ref{thm:AC0} in combination with known results yields an unconditional lower bound on $\cc{AC}^0$-Frege proofs of the PIT axioms.) In particular, we are in the following win-win situation: %(well, win-win in the twisted minds of us complexity theorists, for which lower bounds constitute a ``win'', and lower bounds on lower bounds also constitute a ``win''):

\begin{AC0pcor}
Either 
\begin{itemize}
\item There are polynomial-size $\cc{AC}^0[p]$-Frege proofs of the PIT axioms, in which case \emph{any superpolynomial lower bounds on $\cc{AC}^0[p]$-Frege imply $\cc{VNP}_{\F_p} \neq \cc{VP}_{\F_p}$}, thus explaining the difficulty of obtaining such lower bounds, or

\item There are no polynomial-size $\cc{AC}^0[p]$-Frege proofs of the PIT axioms, in which case we've gotten $\cc{AC}^0[p]$-Frege lower bounds.
\end{itemize}
\end{AC0pcor}

Finally, in Section~\ref{sec:syzygy} we suggest a new framework for proving lower bounds for
the Ideal Proof System which we feel has promise. Along the way, we make precise the difference in difficulty between proof complexity lower bounds (on \I, which may also apply to Extended Frege via Theorem~\ref{thm:EF}) and algebraic circuit lower bounds. In particular, the set of \emph{all $\I$-certificates} for a given unsatisfiable system of equations is, in a certain precise sense, ``finitely generated.'' We suggest how one might take advantage of this finite generation to transfer techniques from algebraic circuit complexity to prove lower bounds on $\I$, and consequently on Extended Frege (since $\I$ p-simulates Extended Frege unconditionally), giving hope for the first time for length-of-proof lower bounds on an algebraic proof system. We hope to pursue this approach in future work.

\subsection{Related Work}

Mention algebraic proof systems (PC, Nullstellensatz, P96/PICM). 

Mention Tzameret/Hrubes proof system for PITs and why it is different.
They basically start with the ring axioms for ring of multivariate polynomials over
$x_1,\ldots,x_n$, and study what equations they can derive from these axioms.
They study families of circuits that have various PIT algs, and see which
families of circuits computing identically zero polynomials have proofs of this fact
in their equational calculus. For example, they show for all circuits computing
polynomials of a restricted form, that any such circuit in this class
computing the identically zero polynoimal has a proof of this fact in their system.
In contrast we want to reason directly about circuits $K$ for solving PIT.

Contrast with Raz--Tzameret

\subsection{Outline}
We start in Section~\ref{sec:general}, by proving several basic facts about \I. We discuss the relationship between \I and previously studied proof systems; in particular, we are able to very quickly and naturally define most of the previously studied algebraic proof systems in terms of familiar circuit-complexity measures on \I. We also highlight several consequences of results from algebraic complexity theory for the Ideal Proof System, such as division elimination \cite{strassenDivision} and the chasms at depth 3 \cite{GKKSchasm,tavenas} and 4 \cite{agrawalVinay,koiranChasm,tavenas}. 

In Section~\ref{sec:VNP}, we prove that lower bounds on \I imply algebraic circuit lower bounds (Theorem~\ref{thm:VNP}). 

In Section~\ref{sec:EF} we introduce our PIT axioms in detail and prove that, if the PIT axioms are efficiently provable in Extended Frege, then EF is p-equivalent to \I. In Section~\ref{sec:AC0p} we show how this proof can be modified to extend to much weaker systems such as $\cc{AC}^0$-Frege and $\cc{AC}^0[p]$-Frege, and discuss in more detail the consequences of this result, as already mentioned briefly above. 

In Section~\ref{sec:syzygy} we suggest a new framework for transfering techniques from algebraic circuit complexity to (algebraic) proof complexity lower bounds.

Finally, in Section~\ref{sec:conclusion} we gather a long list of open questions raised by our work, many of which we believe may be quite approachable.

Appendices~\ref{app:encoding} and \ref{app:background} contain additional details, and Appendix~\ref{app:examples} contains two examples worked out in detail (Tseitin tautologies and the Pigeonhole Principle PHP). 

The remaining appendices contain further fundamental developments; these are relegated to appendices only to focus attention on our main contributions as outlined above. In Appendix~\ref{app:found} we give further basic results on \I, including more algebraic structure on the set of all certificates, and a geometric variant of the Ideal Proof System that may be interesting in its own right. In Appendix~\ref{app:GI} we put forward a suggestive relationship between proof complexity (a la Ideal Proof System) and Graph Isomorphism. In Appendix~\ref{app:RIPS} we discuss a variant of the Ideal Proof System that allows rational functions and division in its certificates.
